A Neural-Network Variational Quantum Algorithm for Many-Body Dynamics

We propose a neural-network variational quantum algorithm to simulate the time evolution of quantum many-body systems. Based on a modified restricted Boltzmann machine (RBM) wavefunction ansatz, the proposed algorithm can be efficiently implemented in near-term quantum computers with low measurement cost. Using a qubit recycling strategy, only one ancilla qubit is required to represent all the hidden spins in an RBM architecture. The variational algorithm is extended to open quantum systems by employing a stochastic Schrodinger equation approach. Numerical simulations of spin-lattice models demonstrate that our algorithm is capable of capturing the dynamics of closed and open quantum many-body systems with high accuracy without suffering from the vanishing gradient (or 'barren plateau') issue for the considered system sizes.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> preamble.tex <==
\usepackage{graphicx,graphics,epsfig,subfigure,times,bm,bbm,amssymb,amsmath,amsfonts,amsthm,mathrsfs,MnSymbol}
\usepackage[matrix,frame,arrow]{xypic}
\usepackage[normalem]{ulem}
\usepackage{slashed}
%\usepackage[c]{hyperref}
\usepackage{color}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
%\usepackage[pdftex]{color}
%\usepackage[hidelinks]{hyperref}
\usepackage[colorlinks=true,
            linkcolor=red,
            urlcolor= darkblue,
            citecolor=blue]{hyperref}
%\usepackage{natbib}
%\usepackage{braket}%Dirac Notation in QM

\usepackage{enumerate}
\usepackage{epstopdf}
%\usepackage{pdfsync}
\usepackage{relsize}

\hyphenpenalty = 900
\linespread{0.956}

%\input{Qcircuit.tex}

\newtheorem{definitionenv}{Definition}
\newtheorem{remarkenv}[definitionenv]{Remark}
\newenvironment{remark}{\begin{remarkenv}\rm}{\end{remarkenv}}

\newtheorem{exampleenv}{Example}
\newenvironment{example}{\begin{exampleenv}\rm}{\end{exampleenv}}


\newtheorem{thm}{Theorem}
\newtheorem{mydef}{Definition}
\newtheorem{col}{Corollary}

\newtheorem{mytheorem}{Theorem}
\newtheorem{mylemma}{Lemma}
\newtheorem{mycorollary}{Corollary}
\newtheorem{myproposition}{Proposition}

\newcommand{\msf}{\mathsf}
\newcommand{\mrm}{\mathrm}
\newcommand{\mbf}{\mathbf}
\newcommand{\mbb}{\mathbb}
\newcommand{\mcal}{\mathcal}




\newcommand{\bes} {\begin{subequations}}
\newcommand{\ees} {\end{subequations}}
\newcommand{\bea} {\begin{eqnarray}}
\newcommand{\eea} {\end{eqnarray}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{black}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

\newcommand{\ph}{\ensuremath{\varphi}}
\newcommand{\eps}{\ensuremath{\varepsilon}} %"nice" epsilon
\newcommand{\prima}[1]{\ensuremath{#1^\prime}} %add a prime to something
\newcommand{\R}{\ensuremath{\mathbb{R}}} %real numbers
\newcommand{\C}{\ensuremath{\mathbb{C}}} %complex numebrs
\newcommand{\Q}{\ensuremath{\mathbb{Q}}} %rational numbers
\newcommand{\Z}{\ensuremath{\mathbb{Z}}} %integers
\newcommand{\N}{\ensuremath{\mathbb{N}}} %natural numbers
\newcommand{\e}{\ensuremath{{e}}} %e:=lim_{n\to\infty}(1+1/n)^n
\newcommand{\ii}{\ensuremath{{i}}}%i:=\sqrt{-1}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}} %absolute value
\newcommand{\norm}[1]{\ensuremath{\left\|#1\right\|}} %norm
\newcommand{\opU}{\ensuremath{{{U}}}}
\newcommand{\opH}{\ensuremath{{{H}}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\dfsh}{\tilde{\mathcal{H}}}
\newcommand{\wt}[1]{\mathrm{wt}(#1)}
\newcommand{\eeq}{\end{equation}}

\newcommand{\upi}{\mathrm{i}}
\newcommand{\upe}{\mathrm{e}}
\newcommand{\upd}{\mathrm{d}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\ignore}[1]{}
\newcommand{\mc}[1]{\mathcal{#1}}

%Greek Letters
\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\d{\delta}
\def\e{\epsilon}
\def\ve{\varepsilon}
\def\z{\zeta}
\def\h{\eta}
\def\t{\theta}
%\def\i{\iota}
\def\k{\kappa}
%\def\l{\lambda}
\def\m{\mu}
\def\n{\nu}
\def\x{\xi}
\def\p{\pi}
%\def\r{\rho}
\def\s{\sigma}
\def\ta{\tau}
\def\u{\upsilon}
\def\ph{\varphi}
\def\c{\chi}
\def\ps{\psi}
\def\o{\omega}

\def\G{\Gamma}
\def\D{\Delta}
\def\T{\Theta}
\def\Lam{\Lambda}
\def\X{\Xi}
\def\P{\Pi}
\def\S{\Sigma}
\def\U{\Upsilon}
\def\Ph{\Phi}
\def\Ps{\Psi}
\def\O{\Omega}

%Some helpful quantum shortcuts
\def\ox{\otimes}
\def\>{\rangle}
\def\<{\langle}
\def\Tr{\mathrm{Tr}}
\def\Pr{\mathrm{Pr}}

\newcommand{\ketbra}[1]{|{#1}\>\<#1|}
\newcommand{\bracket}[1]{\<{#1}|{#1}\>}
\newcommand{\bk}[2]{\<{#1}|{#2}\>}
\newcommand{\ketb}[2]{|{#1}\>\<#2|}
\newcommand{\ketbsub}[3]{|{#1}\>_{#3}\<#2|}
\newcommand{\ident}{\mathbb{I}}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\ket}[1]{|#1\rangle}


\newcommand{\opI}{\ensuremath{{{I}}}}
\newcommand{\opA}{\ensuremath{{{A}}}}
\newcommand{\opB}{\ensuremath{{{B}}}}
\newcommand{\opX}{\ensuremath{{{X}}}}
\newcommand{\opY}{\ensuremath{{{Y}}}}
\newcommand{\opZ}{\ensuremath{{{Z}}}}
\newcommand{\opS}{\ensuremath{{{S}}}}
\newcommand{\ee}{\ensuremath{{e}}} %e:=lim_{n\to\infty}(1+1/n)^n


%\newcommand{\cC}{\mathcal{C}}

%These last ones are due to florjanc@usc.edu, please email me if they conflict with something and you'd like me to revise what I've written to not use them.
\def\lp{\left(}
\def\rp{\right)}
\def\ls{\left[}
\def\rs{\right]}
\def\lb{\left\{}
\def\rb{\right\}}

%By muthukri@usc.edu

\def\dgr{\dagger}

%from Ching-yi
\newcommand{\sfA}{\textsf{A}}
\newcommand{\sfB}{\textsf{B}}
\newcommand{\sfC}{\textsf{C}}
\newcommand{\sfD}{\textsf{D}}
\newcommand{\sfE}{\textsf{E}}
\newcommand{\sfF}{\textsf{F}}
\newcommand{\sfG}{\textsf{G}}
\newcommand{\sfH}{\textsf{H}}
\newcommand{\sfI}{\textsf{I}}
\newcommand{\sfM}{\textsf{M}}
%
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
%\newcommand{\cH}{\mathcal{H}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
%\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}

\newcommand{\rmark}[1]{{\color{red} #1}}
\newcommand{\bmark}[1]{{\color{blue} #1}}
\newcommand{\step}{\tau} %% to replace \mathcal{T}
\DeclareMathOperator*{\bigcdot}{\raisebox{0pt}[\ht\dotbox][\dp\dotbox]{\(\boldsymbol{\cdot}\)}}
